Flexible-Modal Face Anti-Spoofing: A Benchmark

Face anti-spoofing (FAS) plays a vital role in securing face recognition systems from presentation attacks. Benefitted from the maturing camera sensors, single-modal (RGB) and multi-modal (e.g., RGB+Depth) FAS has been applied in various scenarios with different configurations of sensors/modalities. Existing single- and multi-modal FAS methods usually separately train and deploy models for each possible modality scenario, which might be redundant and inefficient. Can we train a unified model, and flexibly deploy it under various modality scenarios? In this paper, we establish the first flexible-modal FAS benchmark with the principle `train one for all'. To be specific, with trained multi-modal (RGB+Depth+IR) FAS models, both intra- and cross-dataset testings are conducted on four flexible-modal sub-protocols (RGB, RGB+Depth, RGB+IR, and RGB+Depth+IR). We also investigate prevalent deep models and feature fusion strategies for flexible-modal FAS. We hope this new benchmark will facilitate the future research of the multi-modal FAS. The protocols and codes are available at https://github.com/ZitongYu/Flex-Modal-FAS.

==> new_command.tex <==

%black
\definecolor{bronze}{rgb}{0.8, 0.5, 0.2}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{brown(web)}{rgb}{0.65, 0.16, 0.16}
\definecolor{cadmiumorange}{rgb}{0.93, 0.53, 0.18}
%for Zitong Yu
\newcommand\Yu[1]{\textcolor{cadmiumorange}{#1}}

%for Wei Peng
\newcommand\pw[1]{\textcolor{bleudefrance}{#1}}
\newcommand\pwC[1]{\textcolor{bleudefrance}{[Wei Peng: #1]}}
%for Xiaobai Li
\newcommand\Li[1]{\textcolor{green}{#1}}

%for Xiaopeng Hong
\newcommand\XP[1]{\textcolor{red}{#1}}
\newcommand\XPC[1]{\textcolor{red}{[Xiaopeng: #1]}}

\newcommand\XPCC[2]{\textcolor{red}{\textit{[Xiaopeng: #1]}\textbf[#2]}}

\newcommand\XPDel[1]{\textcolor{red}{\sout{{#1}}}}

%for Guoying Zhao
\newcommand\Zhao[1]{\textcolor{brown(web)}{#1}}

%updating
\newcommand\up[1]{\textcolor{gray}{#1}}

\def\eg{\emph{e.g.}} \def\Eg{\emph{E.g.}}
\def\ie{\emph{i.e.}}
\def\Ie{\emph{I.e.}}
\def\cf{\emph{c.f.}} \def\Cf{\emph{C.f.}}
\def\etc{\emph{etc.}} \def\vs{\emph{vs.}}
\def\wrt{w.r.t.} 
\def\dof{d.o.f.}
\def\etal{\emph{et al.}}
\def\aka{\emph{a.k.a.}}
